Security Certification in Payment Card Industry: Testbeds, Measurements, and Recommendations

The massive payment card industry (PCI) involves various entities such as merchants, issuer banks, acquirer banks, and card brands. Ensuring security for all entities that process payment card information is a challenging task. The PCI Security Standards Council requires all entities to be compliant with the PCI Data Security Standard (DSS), which specifies a series of security requirements. However, little is known regarding how well PCI DSS is enforced in practice. In this paper, we take a measurement approach to systematically evaluate the PCI DSS certification process for e-commerce websites. We develop an e-commerce web application testbed, BuggyCart, which can flexibly add or remove 35 PCI DSS related vulnerabilities. Then we use the testbed to examine the capability and limitations of PCI scanners and the rigor of the certification process. We find that there is an alarming gap between the security standard and its real-world enforcement. None of the 6 PCI scanners we tested are fully compliant with the PCI scanning guidelines, issuing certificates to merchants that still have major vulnerabilities. To further examine the compliance status of real-world e-commerce websites, we build a new lightweight scanning tool named PciCheckerLite and scan 1,203 e-commerce websites across various business sectors. The results confirm that 86% of the websites have at least one PCI DSS violation that should have disqualified them as non-compliant. Our in-depth accuracy analysis also shows that PciCheckerLite's output is more precise than w3af. We reached out to the PCI Security Council to share our research results to improve the enforcement in practice.

==> pci_requirements.tex <==
{\bf Sazzadur, explain the () around 19, 20 in table 7.}

\begin{table*}[!ht]
\caption{PCI DSS Requirements vs. ASV scanning capabilities. ASV capabilities are derived from the ASV scanning guideline~\cite{DBLP:books/asv/guideline}. ``\LEFTcircle''~means partially covered by external scanning and ``\Circle''~means not covered. The last column shows the corresponding rule indices in Table~\ref{table:experimental-results}.} \label{pci-dssrequirements}
\vspace{-0.1in}
\centering
\small
\begin{tabular}{@{}llll@{}}
\toprule
Goals & Requirements & ASV Scanning \\ \midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Build and Maintain \\ a Secure Network\end{tabular}} & \begin{tabular}[c]{@{}l@{}}1. Install and maintain a firewall configuration to protect cardholder data\end{tabular} & \LEFTcircle \\

& \begin{tabular}[c]{@{}l@{}}2. Do not use vendor-supplied defaults for passwords and security parameters\end{tabular} & \LEFTcircle  \\ \hline
\multirow{2}{*}{Protect Cardholder Data} & 3. Protect stored cardholder data & \Circle \\

& 4. Encrypt transmission of cardholder data across open, public networks & \LEFTcircle  \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Maintain a Vulnerability \\ Management Program\end{tabular}} & 5. Use and regularly update anti-virus software or programs & \LEFTcircle \\

& 6. Develop and maintain secure systems and applications & \LEFTcircle \\ \hline

\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Implement Strong \\ Access Control Measures\end{tabular}} & 7. Restrict access to cardholder data by business need to know & \Circle \\ 

& 8. Assign a unique ID to each person with computer access & \Circle \\

& 9. Restrict physical access to cardholder data & \Circle \\ \hline 

\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Regularly Monitor \\ and Test Networks\end{tabular}} & 10. Track and monitor all access to network resources and cardholder data & \Circle \\

& 11. Regularly test security systems and processes & \Circle \\ \hline

\begin{tabular}[c]{@{}l@{}}Maintain an Information\\  Security Policy\end{tabular}          & 12. Maintain a policy that addresses information security for all personnel  & \Circle \\ \bottomrule
\end{tabular}
\end{table*}

==> screenshots.tex <==
\begin{figure*}[!ht]
    \centering
    \fbox{\includegraphics[width=0.35\textwidth]{main_page.png}}
    \caption{Homepage of www.rwycart.com.}
    \label{fig:homepage}
\end{figure*}

\begin{figure*}[!ht]
    \centering
    \fbox{\includegraphics[width=0.35\textwidth]{customer_login.png}}
    \caption{Customer login page of www.rwycart.com.}
    \label{fig:customer-login}
\end{figure*}

% \begin{figure*}[!ht]
%     \centering
%     \includegraphics[width=0.80\textwidth]{admin_login.png}
%     \caption{Administrator login page of www.rwycart.com.}
%     \label{fig:my_label}
% \end{figure*}
